Learning trends of COVID-19 using semi-supervised clustering

A finite mixture model is used to learn trends from the currently available data on coronavirus (COVID-19). Data on the number of confirmed COVID-19 related cases and deaths for European countries and the United States (US) are explored. A semi-supervised clustering approach with positive equivalence constraints is used to incorporate country and state information into the model. The analysis of trends in the rates of cases and deaths is carried out jointly using a mixture of multivariate Gaussian non-linear regression models with a mean trend specified using a generalized logistic function. The optimal number of clusters is chosen using the Bayesian information criterion. The resulting clusters provide insight into different mitigation strategies adopted by US states and European countries. The obtained results help identify the current relative standing of individual states and show a possible future if they continue with the chosen mitigation technique

==> application.tex <==
\section{Application}
\label{sect.appl}
In this section, the algorithm MMN-VarSel is validated on real-life data in comparison with the same procedures considered in Section~\ref{sect.exp}. The Landsat Satellite data set is publicly available at the UCI repository \citep{Dua:2019} and contains image data generated by the Landsat Multi-Spectral Scanner. Each observation consists of four digital images ($d = 4$) of the same scene provided in different spectral bands. Every image is represented by nine pixels ($p = 9$) with recordered intensity values ranging from 0 (black color) to 255 (white color). Hence, in the training portion of the data, there are 4,435 matrices of dimensions $9 \times 4$ representing six types of soil: $1072$ red, $479$ cotton crop, $961$ grey, $415$ damp grey, $470$ vegetation stubble, and $1038$ very damp grey. The objective of our analysis is to find the most accurate membership prediction. It is known in the literature that the full version of the data set is challenging for clustering. Hence, we consider a reduced version of the data first and then investigate the performance of the competing procedures on the entire set. For the reduced set of data, three soil types have been selected: red, grey, and very damp grey.  The performance of the clustering procedures can be evaluated based on ARI values and percentage of correctly classified observations that are presented in Table~\ref{table.appl}. As we can see, MMN-VarSel outperforms the competitors in both settings. For the reduced data set, 86.1\% of data points are correctly classified and ARI value is 0.655. The closest competitors are {\it VarSelLCM} and {\it SelvarMix} with 67\% and 65.3\% of observations correctly assigned to their classes. The worst performance with 52\% is shown by MMN. The full set of data is more challenging but MMN-VarSel still shows reasonable performance with 74.8\% of data classified correctly and ARI equal to 0.594. The alternative approaches exhibiting the closest performance are MMN (70.6\%) and {\it VarSelLCM} (69.7\%).
\begin{table*}[t]
  \caption{Results obtained for for the reduced and full Satellite data}
  \vspace{-0.1in}
	\label{table.appl}
\centering
\begin{tabular}{c}
%	\begin{minipage}{0.5\linewidth}
			\begin{tabular}{ l|c|c|c|c|c|c} 
			\hline
		&  & MMN  & MMN-VarSel & {\it SelvarMix} & {\it sparcl} & {\it VarSelLCM}\\
			\hline
	Satellite  & ARI & 0.391 & \textbf{0.655}  &  0.492 & 0.334 & 0.362\\
			\cline{2-7}
	reduced		& \% & 52.0  &\textbf{86.1} & 65.3 & 61.1 & 67.0\\
%			\hline
%		\end{tabular}
%	\end{minipage} \\
%	\\
%	\begin{minipage}{0.5\linewidth}
%			\begin{tabular}{ c|c|c|c|c|c} 
%			\hline
%			& & MMN  & MMN-VarSel &SelvarMix& sparcl &VarSelCM\\
			\hline
	Satellite		& ARI &  0.581& \textbf{0.594}  & 0.433 &  0.292 & 0.460\\
			\cline{2-7}
	full		& \% &  70.6 &\textbf{74.8} & 56.6 & 47.5 & 69.7\\
			\hline
		\end{tabular}
%		\caption{Comparing variable
%		selection methods on satellite data 2}
%	\label{tab:5}
%	\end{minipage} 
\end{tabular}
\end{table*}
\begin{table}
  \caption{Classification agreement matrices for the reduced Satellite data set}
  \label{table.classred}
      \vspace{-0.1in}
	\centering
	\resizebox{0.99\columnwidth}{!}
	{\begin{tabular}{| l|c c c|c c c|c c c|c c c|c c c|} 
			\hline
			&	\multicolumn{3}{c|}{MMN} &	\multicolumn{3}{c|}{MMN-VarSel} &	\multicolumn{3}{c|}{{\it SelvarMix}}&\multicolumn{3}{c|}{{\it sparcl}} &	\multicolumn{3}{c|}{{\it VarSelLCM}}\\
			\hline
			Soil type & 1  &2 & 3 & 1  &2 & 3 & 1   &2 & 3 &
				1 & 2 & 3 & 1  &2 & 3 \\
			\hline
			
			 1. Red soil   & \textbf{477} & 595 &0  &  \textbf{1050}&22&0&\textbf{963}&109&0&\textbf{381} &569&122&\textbf{499}& 573&0\\
			
			2. Grey soil & 0  &\textbf{131}& 830 &  34&\textbf{923} &4&0&\textbf{151}&810&334&\textbf{621}&6&124&\textbf{837}&0\\
			
			3. Very damp grey soil &  0 &49&\textbf{989}& 51&316&\textbf{671}&0&148&\textbf{890}&164&1& \textbf{873}&311&6&\textbf{721}\\
			\hline
	\end{tabular}}
\end{table}

Tables~\ref{table.classred} and \ref{table.classfull} provide classification agreement results between the assignments based on the soil type and those obtained by the five methods under consideration. As we can see, MMN-VarSel performs rather well. The only substantial difficulty it faces is related to classifying very damp grey soil images as there are 316 of them incorrectly assigned to the grey soil class. At the same time, we can observe that all competing methods encounter even more severe challenges with clustering observations correclty. The classification agreement matrices corresponding to the full data set are provided in Table~\ref{table.classfull}. As we can see, MMN-VarSel performs well, with the most uncertainty associated with grey and dump grey soil. Many observations from these two classes are assigned to cluster 6. However, it can be observed that the alternative methods have more severe challenges with the clustering assignment.

\begin{table}
    \caption{Classification agreement matrices for the full Satellite data set}
    \label{table.classfull}
    \vspace{-0.1in}
\resizebox{\columnwidth}{!}
{\begin{tabular}{c}
	\begin{minipage}{1.25\linewidth}
		\begin{tabular}{| l|c c c c c c|c c c c c c|c c c c c c|} 
	
		\hline
		&	\multicolumn{6}{c|}{MMN}&	\multicolumn{6}{c|}{MMN-VarSel} &	\multicolumn{6}{c|}{{\it SelvarMix}}\\
		\hline
		Soil type  & 1  &2 & 3 &4 &5 &6& 1  &2 & 3 &4 &5 &6& 1  &2 & 3 &4 &5 &6 \\
		\hline
		
	 1. Red soil &\textbf{638}&0&2&419&13&0 &\textbf{1051}&0&0&19&0&2&\textbf{938}&0&0&12&0&122\\

	2. Cotton crop &0&\textbf{337}&0&0&142&0 &1&\textbf{336}&1&111&12&18&0&\textbf{302}&0&176&1&0\\
	
		3. Grey soil &55&0&\textbf{855}&0&47& 4&53&0 &\textbf{685}&25&0&198&0&0&\textbf{723}&21&0&217\\

		4. Damp grey soil &12&0&141&\textbf{0}&56&206 &17&1&80&\textbf{24}&6&287&0&0&283&\textbf{41}&9&82\\

		5. Soil with vegetation stubble &28&0&0&0&\textbf{386}&56 &26&2&2&103&\textbf{297}&40&7&7&6&46&\textbf{318}&86\\
		
		6. Very damp grey soil &0&0&48&0&74&\textbf{916}&1&0&17&24&75&\textbf{922}&0&0&758&16&77&\textbf{187}\\
		\hline
		\end{tabular}
	\end{minipage} 
\\
	\begin{minipage}{1.25\linewidth}
	\begin{tabular}{| l| c c c c c c|c c c c c c|} 
%		\hline
		&\multicolumn{6}{c|}{{\it sparcl}} &	\multicolumn{6}{c|}{{\it VarSelLCM}}\\
		\hline
		Soil type  & 1  &2 & 3 &4 &5 &6 & 1  &2 & 3 &4 &5 &6\\
		\hline
	   1. Red soil & \textbf{244}&0&419&239&2&168&\textbf{519}&0&25&344&184&0\\
		2. Cotton crop &	0&\textbf{356}&0&5&87&31&0&\textbf{344}&5&16&119&0\\
	3. Grey soil &	363 &0&\textbf{583}&15&0&0&0&0&\textbf{828}&131&2&0\\
	4.  Damp grey soil &	127&0&36&\textbf{221}&0&31&0&0&58&\textbf{321}&9&27\\
	5. Soil with vegetation stubble &	16&0&0&35&\textbf{282}&133&0&0&0&66&\textbf{358}&37\\
	6. Very damp grey soil & 61&0&0&349&10&\textbf{618}&0&0&6&278&32&\textbf{722}\\
		\hline
	\end{tabular}
\end{minipage}
\end{tabular}}
\end{table}



%To validate the proposed method, we have done experiments on tow datasets: (1) the dataset 1 consisting of all images of the red soil, grey soil images and very damp grey soil of the training set; (2) the dataset 2 is entire training set with 4435 observations. The ARIs' and MCRs', and confusion matrix of all methods are recorded in tables $\ref{tab:4}$, $\ref{tab:5}$, $\ref{table:7}$ and $\ref{table:8}$. They illustrates that MMN-VarSel obtains the best classification results. Moreover, in the dataset 1 the MMN-VarSel selects all variables except the eighth on the first row and the in the dataset entire fourth row is selected. They illustrate that only one of digital image can represent the data better than all four images together does. Consequently, the proposed models select the most relevant variables and gives the best classification accuracy. 





